The Permute-and-Flip Mechanism is Identical to Report-Noisy-Max with Exponential Noise

The permute-and-flip mechanism is a recently proposed differentially private selection algorithm that was shown to outperform the exponential mechanism. In this paper, we show that permute-and-flip is equivalent to the well-known report noisy max algorithm with exponential noise.

==> applications.tex <==
McKenna and Sheldon \cite{paf} analyzed the privacy and utility properties of Permute-and-Flip. By our equivalence, these results carry over to Report Noisy Max with Exponential Noise. However, some of these results are substantially simpler to prove directly, as we now show.

We start by proving the privacy of Report Noisy Max with Exponential Noise. This proof is a simple exercise \cite{homework}, whereas the privacy analysis of Permute-and-flip is somewhat involved.

\begin{proposition}\label{prop:dp}
Report Noisy Max with Exponential Noise (Algorithm \ref{alg:nm}) is $\varepsilon$-differentially private.
\end{proposition}
\begin{proof}
 Let $q$ be the quality function with sensitivity $\Delta$ and set of outcomes $\Omega = \{ \omega_1, \cdots, \omega_k \}$.
 Let $D_1$ and $D_2$ be neighbouring datasets and let $\omega \in \Omega$ be an arbitrary output.
 As in Algorithm \ref{alg:nm}, sample $v_j^b \gets q(D_b,\omega_j)+\expo(\frac{\varepsilon}{2\Delta})$ for all $\omega_j \in \Omega$ and $b \in \{1,2\}$. For notational convenience, denote $\xi_j^b = v_j^b - q(D_b,\omega_j)$. Note that all the $\xi_j^b$ random variables are distributed according to $\expo(\frac{\varepsilon}{2\Delta})$.
 Now
 \begin{align*}
     \pr{}{M(D_1) = \omega_i} &= \pr{}{v_i^1 \ge \max_j v_j^1 }\\
     &= \pr{}{\xi_i^1 \ge \max_j q(D_1, \omega_j) - q(D_1,\omega_i) + \xi_j^1}\\
     &= \pr{}{\xi_i^2 \ge \max_j q(D_1, \omega_j) - q(D_1,\omega_i) + \xi_j^2}\\
     &\le \pr{}{\xi_i^2 \ge \max_j q(D_2, \omega_j) - q(D_2,\omega_i) -2\Delta + \xi_j^2}\tag{since $q(D_2, \omega_j) - q(D_2,\omega_i) -2\Delta \le q(D_1, \omega_j) - q(D_1,\omega_i)$}\\
     &\le e^{2\Delta \cdot \frac{\varepsilon}{2\Delta}} \cdot \pr{}{\xi_i^2 \ge \max_j q(D_2, \omega_j) - q(D_2,\omega_i) + \xi_j^2}\tag{since $\pr{}{\xi \ge x - 2\Delta} \le e^{2\Delta \lambda} \cdot \pr{}{\xi \ge x}$ whenever $\xi \gets \expo(\lambda)$}\\
     &= e^\varepsilon \cdot \pr{}{M(D_2)=\omega_i}.
 \end{align*}
\end{proof}

With this simplified proof in hand, we can also provide an improve privacy result. For this, we introduce a refined version of differential privacy:
\begin{definition}[Bounded Range \cite{boundedrange,ddr}]
    A randomized algorithm $M$ with discrete output space $\Omega$ satisfies $\varepsilon$-bounded range privacy if, for all inputs $D_1$ and $D_2$ differing on the addition or removal of single individual, there exists $t \in \mathbb{R}$ such that \[\forall \omega \in \Omega ~~\qquad~~ e^{t-\varepsilon} \le \frac{\pr{}{M(D_1)=\omega}}{\pr{}{M(D_2)=\omega}} \le e^t.\]
\end{definition}

Note that $\varepsilon$-bounded range privacy implies $\varepsilon$-differential privacy, but $\varepsilon$-differential privacy only implies $2\varepsilon$-bounded range. As we discuss later, bounded range privacy is known to give better bounds for \emph{concentrated differential privacy} than pure differential privacy does.

We can prove bounded range privacy and we can also replace sensitivity with a more refined measure. 

\begin{proposition}\label{prop:br}
Report Noisy Max with Exponential Noise (Algorithm \ref{alg:nm}) is $\varepsilon$-bounded range private. This also holds if we replace the sensitivity $\Delta$ with the parameter
\begin{equation}
    \hat\Delta := \sup_{D_1, D_2} ~~ \frac12 \left( \max_j q(D_1,\omega_j)-q(D_2,\omega_j) \right) - \frac12 \left( \min_j q(D_1,\omega_j)-q(D_2,\omega_j) \right), \label{eq:senshat}
\end{equation}
where the supremum is taken over all pairs of datasets differing on the records of one person.
\end{proposition}
\begin{proof}
 As in the proof of Proposition \ref{prop:dp}, we have
 \begin{align*}
     &\!\!\!\frac{\pr{}{M(D_1)=\omega_i}}{\pr{}{M(D_2)=\omega_i}} \\
     &= \frac{\pr{}{\xi_i^2 \ge \max_j q(D_1,\omega_j)-q(D_1,\omega_i)+\xi_j^2}}{\pr{}{\xi_i^2 \ge \max_j q(D_2,\omega_j)-q(D_2,\omega_i)+\xi_j^2}}\\
     &= \frac{\ex{}{\min\{1,\exp(-\frac{\varepsilon}{2\Delta} \cdot \max_{j\ne i} q(D_1,\omega_j)-q(D_1,\omega_i)+\xi_j^2)}}{\ex{}{\min\{1,\exp(-\frac{\varepsilon}{2\Delta} \cdot \max_{j\ne i} q(D_2,\omega_j)-q(D_2,\omega_i)+\xi_j^2)}}\\
     &\le \exp\left(\frac{\varepsilon}{2\Delta} \cdot ( \max_{j_2 \ne i} q(D_2,\omega_{j_2})-q(D_2,\omega_i) - \max_{j_1 \ne i} q(D_1,\omega_{j_1}) + q(D_1,\omega_i))\right)\\
     &\le \exp\left(\frac{\varepsilon}{2\Delta} \cdot ( \max_{j_2 \ne i} q(D_2,\omega_{j_2}) - \max_{j_1 \ne i} q(D_1,\omega_{j_1}) + \max_{j_3} q(D_1,\omega_{j_3})-q(D_2,\omega_{j_3}))\right).
 \end{align*}
 Similarly, \[\frac{\pr{}{M(D_1)=\omega_i}}{\pr{}{M(D_2)=\omega_i}} \!\ge\! \exp\!\left(\!\frac{\varepsilon}{2\Delta} \!\cdot\! ( \max_{j_2 \ne i} q(D_2,\omega_{j_2}) \!-\! \max_{j_1 \ne i} q(D_1,\omega_{j_1}) \!+\! \min_{j_3} q(D_1,\omega_{j_3})\!-\!q(D_2,\omega_{j_3}))\!\right).\]
 This means we have bounded range privacy with parameter \[\frac{\varepsilon}{2\Delta} \left( \max_j q(D_1,\omega_j) - q(D_2,\omega_j) - \min_{j'} q(D_1,\omega_{j'})-q(D_2,\omega_{j'})\right) \le \varepsilon,\] as required.
\end{proof}

Another refined notion of differential privacy is \emph{concentrated differential privacy} \cite{dr16}:
\begin{definition}[Concentrated Differential Privacy \cite{bs16}]
A randomized algorithm $M$ satisfies $\rho$-concentrated differential privacy ($\rho$-CDP) if, for all datasets $D_1$ and $D_2$ differing on the data of a single person, we have $\dr{\alpha}{M(D_1)}{M(D_2)} \le \alpha \cdot \rho$ for all $\alpha \in (1,\infty)$.
Here $\dr{\alpha}{X}{Y} := \frac{1}{\alpha-1} \log \left(\sum_\omega \pr{}{X=\omega}^\alpha \cdot \pr{}{Y=\omega}^{1-\alpha}\right)$ is the R\'enyi divergence of order $\alpha$.
\end{definition}

It is known that $\varepsilon$-differential privacy implies $\frac12\varepsilon^2$-CDP \cite{bs16}. However, $\varepsilon$-bounded range privacy implies $\frac18 \varepsilon^2$-CDP \cite[Lemma 3.2]{br-cdp}.
Combining Proposition \ref{prop:br} with this conversion yields the following improved bound for selection with concentrated differential privacy.

\begin{corollary}
Report Noisy Max with Exponential Noise (Algorithm \ref{alg:nm}) satisfies $\frac18 \varepsilon^2 $-CDP. This also holds if we replace the sensitivity with the parameter $\hat\Delta$ given in Equation \ref{eq:senshat}.
\end{corollary}

In addition to the above privacy analysis, our characterization also allows us to obtain simple utility bounds (these are known \cite{paf} and also hold for the exponential mechanism \cite{exponentialMechanism,bassily2021algorithmic}, but we provide a simple self-contained proof):

\begin{proposition}
Let $D$ be a dataset and let $q$ be a quality function with sensitivity $\Delta$ and set of outcomes $\Omega = \{\omega_1, \cdots, \omega_k\}$. Fix $\varepsilon>0$. Let $M(D)$ denote Algorithm \ref{alg:nm} run with these inputs. Then
\begin{equation}
    \ex{}{q(D,\omega_{M(D)})} \ge \max_i q(D,\omega_i) - \frac{2\Delta}{\varepsilon} \log k
\end{equation}
and, for all $\beta > 0$
\begin{equation}
    \pr{}{q(D,\omega_{M(D)}) \ge \max_i q(D,\omega_i) - \frac{2\Delta}{\varepsilon} \log\left(\frac{k}{\beta}\right)} \ge 1 - \beta.
\end{equation}
\end{proposition}
\begin{proof}
 Let $i_* = \argmax_i q(D,\omega_i)$.
 Let $\xi_1, \cdots, \xi_k \gets \expo(\frac{\varepsilon}{2\Delta})$ denote the noise values -- i.e., $\xi_i = v_i - q(D,\omega_i)$.
 Since $M(D) = \argmax_i q(D,\omega_i)+\xi_i$, we have \[q(D,\omega_{M(D)}) + \xi_{M(D)} \ge \max_i q(D,\omega_i) + \xi_i \ge q(D,\omega_{i_*}) + \xi_{i_*} = \max_i q(D, \omega_i) + \xi_{i_*}.\]
 We have $\ex{}{\xi_{i_*}}=\frac{2\Delta}{\varepsilon}$ and \[\ex{}{\xi_{M(D)}} \le \ex{}{\max_i \xi_i} = \int_0^\infty \pr{}{\max_i \xi_i \ge t} \mathrm{d}t \le \int_0^\infty \min \{1, k \cdot e^{-\frac{\varepsilon}{2\Delta} t} \} \mathrm{d}t = \frac{2\Delta}{\varepsilon} \left( 1 + \log k \right).\]
 Combining these yields the first part of the result: \[\ex{}{q(D,\omega_{M(D)})} \ge \max_i q(D,\omega_i) + \ex{}{\xi_{i_*}} - \ex{}{\xi_{M(D)}} \ge \max_i q(D,\omega_i) - \frac{2\Delta}{\varepsilon} \log k.\]
 To obtain the second part, we use the fact that $\xi_{i_*} \ge 0$ and $\pr{}{\xi_{M(D)} \ge t} \le \pr{}{\max_i \xi_i \ge t} \le k \cdot e^{-\frac{\varepsilon}{2\Delta} t}$ for all $t \ge 0$.
\end{proof}

==> otherclaims.tex <==
\begin{itemize}
\item DP Book, page 37, lines 3-4 claims that max noisy value in noisy max can be released
\item DP Book, Theorem 3.13, the output distribution of the one-sided noisy max is the exponential mechanism. (instead it is gumbel noise)
\end{itemize}
